Faster Linear-Size And-Or Path and Adder Circuits

We consider the fundamental problem of constructing fast and small circuits for binary addition. We propose a new algorithm with running time $\mathcal O(n \log_2 n)$ for constructing linear-size $n$-bit adder circuits with a significantly better depth guarantee compared to previous approaches: Our circuits have a depth of at most $\log_2 n + \log_2 \log_2 n + \log_2 \log_2 \log_2 n + \text{const}$, improving upon the previously best circuits by [12] with a depth of at most $\log_2 n + 8 \sqrt{\log_2 n} + 6 \log_2 \log_2 n + \text{const}$. Hence, we decrease the gap to the lower bound of $\log_2 n + \log_2 \log_2 n + \text{const}$ by [5] significantly from $\mathcal O (\sqrt{\log_2 n})$ to $\mathcal O(\log_2 \log_2 \log_2 n)$. Our core routine is a new algorithm for the construction of a circuit for a single carry bit, or, more generally, for an And-Or path, i.e., a Boolean function of type $t_0 \lor ( t_1 \land (t_2 \lor ( \dots t_{m-1}) \dots ))$. We compute linear-size And-Or path circuits with a depth of at most $\log_2 m + \log_2 \log_2 m + 0.65$ in time $\mathcal O(m \log_2 m)$. These are the first And-Or path circuits known that, up to an additive constant, match the lower bound by [5] and at the same time have a linear size. The previously fastest And-Or path circuits are only by an additive constant worse in depth, but have a much higher size in the order of $\mathcal O (m \log_2 m)$.

==> glossary.tex <==
\provideglossaryentry{natural numbers}
{
 name={\ensuremath{\N}},
 description={Set of natural numbers including $0$. \cref{sec:functions}},
 sort={natural numbers}
}

\provideglossaryentry{flodd}
{
 name={\ensuremath{\flodd(x)}},
 description={Given $x \in \R$, we write $\flodd(x) = \max \set{y \in \Z \where y \text{ odd}, y \leq x}$. \cref{def-flodd}},
 sort={flodd x}
}


==> settings/shortcref.tex <==
\makeatletter
% Macros adapted from this post: https://stackoverflow.com/a/964813/2747160
% Stores chip attribute:
%  #1: type of attribute (eg. name or technology)
%  #2: identificator of chip (ie. key in lookup table)
%  #3: attribute value
% Example: \registerShorthand{codename}{isztop}{Malygos}
% registers the "codename"-attribute of chip "isztop".
\newcommand\registerShorthand[2]{%
 \@namedef{shorthand-#1}{#2}%
}
% Access (previously) stored chip attribute:
%  #1: type of attribute (eg. name or technology)
%  #2: identificator of chip (ie. key in lookup table)
% Evaluates to the stored value if any or a default placeholder.
\newcommand\getShorthand[1]{%
  \@ifundefined{shorthand-#1}{%
   UNDEFINED%
  }{%
    \@nameuse{shorthand-#1}%
  }%
}

\registerShorthand{Definition}{Def.}
\registerShorthand{Section}{Sec.}
\registerShorthand{Theorem}{Thm.}
\registerShorthand{Proposition}{Prop.}
\registerShorthand{Lemma}{Lem.}
\registerShorthand{Corollary}{Cor.}
\registerShorthand{Remark}{Rem.}
\registerShorthand{Example}{Ex.}
\registerShorthand{Observation}{Obs.}
\registerShorthand{Claim}{Cl.}
\registerShorthand{Table}{Table}
\registerShorthand{Algorithm}{Alg.}
\registerShorthand{line}{l.}

\newcommand{\short}[1]{
 \@setnamecref{cref}{#1}{}{\expandafter\getShorthand}
}
\makeatother
\newcommand{\shortcref}[1]{\text{\short{#1}}\labelcref{#1}}

